Fairness Implications of Encoding Protected Categorical Attributes

Past research has demonstrated that the explicit use of protected attributes in machine learning can improve both performance and fairness. Many machine learning algorithms, however, cannot directly process categorical attributes, such as country of birth or ethnicity. Because protected attributes frequently are categorical, they must be encoded as features that can be input to a chosen machine learning algorithm, e.g.\ support vector machines, gradient boosting decision trees or linear models. Thereby, encoding methods influence how and what the machine learning algorithm will learn, affecting model performance and fairness. This work compares the accuracy and fairness implications of the two most well-known encoding methods: \emph{one-hot encoding} and \emph{target encoding}. We distinguish between two types of induced bias that may arise from these encoding methods and may lead to unfair models. The first type, \textit{irreducible bias}, is due to direct group category discrimination, and the second type, \textit{reducible bias}, is due to the large variance in statistically underrepresented groups. We investigate the interaction between categorical encodings and target encoding regularization methods that reduce unfairness. Furthermore, we consider the problem of intersectional unfairness that may arise when machine learning best practices improve performance measures by encoding several categorical attributes into a high-cardinality feature.

==> content/miscellaneous.tex <==
Thus, following the open data for reproducible research guidelines described in \cite{turing} and for measuring the performance of the proposed methods, we have used a synthetic dataset for a more theoretical evaluation together with 4 open-source datasets for an empirical comparison. The selected datasets are:

\begin{itemize}
    \item \textit{Compass Data}: Propublica...... These dataset has one high cardinality categorical feature that is the protected attribute. It's an intersectional fairness created by concatenating "ethnicity" and "marital status"
    \item \textit{The StackOverflow 2018 Developer survey}\label{dataset:StackOverflow2018} \cite{so2018} is a data set with only five categorical features, namely country, employment status, formal education, developer type, and languages worked. The target variable is the annual salary of the user. 
    
    \item \textit{The StackOverflow 2019 Developer survey}\label{dataset:so2019} \cite{so2019} is a data set with a single categorical feature (country), few numerical features (working week hours, years of coding, and age), and a long-tailed target variable (salary).
    
    \item \textit{Kickstarter Projects} \cite{ksdata} is a data set with crowd-funding projects where the goal is to predict what is the funding goal of each project. The categorical features are the crowd-funding type, the country, the state, and the currency.
    
    \item \textit{Medical Payments}\cite{medical_payments} \label{dataset:medical} is a data set with information about the price of a medical treatment. The dataset consists of 10 categorical features containing information about the state, city, zip code, country, physician type, physician country, the payment method, and its nature.
\end{itemize}

The datasets have undergone a minimal curation process, where miscellaneous features are removed and only the columns that are considered meaningful and informative for the modeling of the problem are kept. 

For the synthetic dataset, we have used the Cauchy distribution in Eq.~\ref{eqn:cauchy} to create a target distribution with long tails. The Cauchy distribution is parameterized by $t$ and $s$, being $t$ the location parameter and $s$ the scale parameter as follows,

\begin{equation}
\label{eqn:cauchy}
    Cauchy(x;t,s) = \frac{1} {s\pi(1 + ((x - t)/s)^{2})}.
\end{equation}

Next,we have created two features, $x_1$ and $x_2$ accordingly,

$$
c_i \sim U(0, 100), \quad x_1 \sim Cauchy(x;c_i,1), \quad x_2 \sim Cauchy(x;c_i,2),
$$

where $\epsilon \sim N(0, 1)$ is sampled from a normal distribution and $x_1$ and $x_2$ are generated sampling from the Cauchy density function. Both features even if numerical are then treated as categorical variables. The corresponding regression target is generated as

$$
y = x_1 + x_2 + \epsilon
$$



A common issue when using target-based encodings such as mean encoding or the quantile encoding is not having enough statistical mass for some of the encoded categories. And, therefore, this creates features that are very close to the target label. Thus, they are prone to over-fitting. A possible solution is to regularize the target encoding feature using additive smoothing, as in \cite{mestimator,wiki:additive-smoothing}. To do so, we compute the target encoding statistic using the following equation: 


%\subsubsection{Regularization}\label{sec:regularization}

\begin{equation}
\label{eqn:mestimate}
\tilde{x}^{(j)}_i = \frac{\hat{x}^{(j)}_i \cdot n_i + q_p(\{y\}) \cdot m }{n_i + m}
\end{equation}
where,
\begin{itemize}
    \item $\tilde{x}^{(j)}_i$ is the target statistic applied to the value corresponding to element $x_i^{(j)}$.
    \item $\hat{x}^{(j)}_i$ is the non-regularized target statistic.
    \item $n_i$ is the number of samples sharing the same value as $x_i^{(j)}$.
    \item $m$ is a regularization parameter, the higher $m$ the more the group statistics tends to be the global one. It can be interpreted as the number of samples needed to have the local contribution (target statistic of the category) equal to the global contribution (global statistic).
\end{itemize}

The rationale of Equation \ref{eqn:mestimate} is that, if a class has very few samples, $n_i \ll m$ then the target statistic  will basically be the global statistic, $\tilde{x}^{(j)}_i \approx q_p(\{y\})$. If a class has a large number of samples, $n_i \gg m$ and $\tilde{x}^{(j)}_i \approx \hat{x}_i^{(j)}$ then the class statistic will have more weight than the global statistic. As a result, the Target Encoder transformation of categorical features has one main hyperparameter that can be tuned to increase, adjust, and modify the type of encoding: $m$ is a regularization hyperparameter. The range of this parameter is $m \in [0, \infty)$. For the specific case where $m=0$, there is no regularization. The larger the value of $m$, the most the Target Encoder features tends to the global target statistic.

An alternative encoding technique is Label/Ordinal Encoding \cite{ordinal} which uses a single column of integers to represent the different categorical values. These are assumed to have no true order and integers are selected at random. This encoding handles the problem of the high dimensional encoding found in One Hot Encoding but imposes an artificial order on the categories. This makes it harder for the model to extract meaningful information. For example, when using a linear model, this effect prevents the algorithm from assigning a high coefficient to this feature.




Anti-discrimination laws \cite{gdpr} prohibits unfair treatment of individuals based on specific traits, also
called sensitive or protected attributes (e.g., sexual orientation, ethnicity, marital status). These laws typically distinguish between two different notions of unfairness \cite{Barocas2016BigDD} namely, \textit{disparate treatment} and \textit{disparate impact}.  More specifically, there is disparate treatment with respect to a given sensitive attribute if the missclasification rates for groups of people have different values of that sensitive attribute.

\cite{zafar2017fairness}, mitigate disparate treatment fairness by developing a decision boundary-based classifiers, which can be easily incorporated into their formulation as convex-concave constraints. In order to avoid high cardinality scenarios, they simplify by only consider a subset of offenders whose race was either black or white. While in our case we deal with all the different types of ethinicity up to 9 distinct values and increase the cardinality of problem by tackling intersectional fairness. 

This notion can be stated in a very intuitive way: \textit{two similar persons should not be treated differently solely because of a difference in a protected attribute}.



During modeling stage of a machine learning (ML) prediction problem, there is the need of feeding the model with meaningful features that describe the problem in a relevant way. That is why the steps of data preparation and feature engineering are crucial in any ML project~\cite{mle,hands-on,quantile2021}. With the recent amount of available data, there is an inevitable increment of protected and sensitive features available for modeling purposes. For the specific case of protected categorical variables this increment can have two different effects: (a) they start being more used and their predictive power can be highly relevant in many cases (b) is not trivial to determine which attributes are protected/sensitive or other attributes correlate with them. When facing both scenarios, the problem of representing categorical features effectively, efficiently and in a non-discriminatory way gains importance for the field of responsible AI CITE.

Encoding categorical features to numerical has been extensively studied in the literature with the statistical methods firstly introduced in the mid 1950's \citep{high-cardinality-categorical,quantile2021,statisticallearning}, since then, they have increasingly been applied in a plethora of machine learning applications, with two of them being most widely used: One Hot Encoding and statistical Target Encoders \cite{quantile2021,category_encoders,catboost-encoder,pargent2021regularized}.

One Hot Encoding produces orthogonal and equidistant vectors for each category \cite{one_hot,natureOHE}. However, when dealing with high cardinality categorical features, one hot encoding suffers from several shortcomings \cite{catFeatBayesian}: (a) the dimension of the input space increases with the cardinality of the encoded variable, (b) the created features are sparsely populated leaving many corresponding dimensions nearly unused, and (c) One Hot Encoding does not handle new and unseen categories \cite{quantile2021}.

Target Encoding (or mean encoding)\cite{quantile2021,high-cardinality-categorical,pargent2021regularized} works as an effective solution to overcome the issue of high cardinality of the categorical variable. In target encoding, categorical features are replaced with the mean target value of each respective category.
%This method is the industry standard for cases with high cardinality of categorical features. 
Target encoding methods have become an industry standard for high-cardinality categorical data \citep{quantile2021,pargent2021regularized,target_embedding} with algorithmic procedures being implemented in many open source packages \cite{sktools,category_encoders}. One of the most common one's is  \textit{category encoders} a Python package. It achieves up to 1 million downloads per month.  \footnote{\url{https://pepy.tech/project/category_encoders}} %demonstrating the frequent usage of encoding methods in real-world applications.
It's even the default encoding method in some high-performance open source software implementations such as \textit{catboost} \cite{catboost-encoder,hancock2020catboost,dorogush2018catboost} that reaches an historical total download of 33 millions.

\textbf{Steffen: here is a gap. What is the story of going from the usage of encoders to fairness? The fairness metric is then already a very specific choice, that can but need not appear in the intro}
\gourab{Here, we can talk about imbalance in datasets. Target encodings of sensitive attributes in imbalanced datasets will introduce less representative and biased encodings even prior to the decision-making process which are found to bring unfairness in outcomes.}
 Encoding protected attributes posses a fairness risk as once converted to numerical features, traditional ML pipelines  will fit a established optimization algorithm whose loss function is fairness ignorant. Correct feature engineering of protected attributes can lead to avoid unwanted pre-processing  bias in the machine learning project life cycle. 

\textbf{Steffen: In the remainder of the section we build up requirements, which is good. However, we do so in a somewhat ad-hoc way rather than saying: `here is an example use case....This use case has the 4 requirements....'}

%In this work we focus particularly on target encoding regularization methods as a bias mitigation strategy in the pre-processing step.

The main drawback of Target Encoding appears when categories with few (even only one) samples are replaced by values close to the desired target. This biases the model to over-trust the target encoded feature and makes it prone to over-fitting. From a fairness perspective target encoding methods lead to map numerically  categories with a few samples, with a statistic that is not be representative of the category group but only from a few instances.

For example, when encoding the ethnic of recidivism risk (the risk that a criminal defendant will re-offend), highly represented ethnicity in the train data-set will have a rich representative target encoding while vaguely represented ethnicity that might only have a few instances in the data-set will be represented by a minority of training instances. For a new user, from one of the less statistically represented countries, might be at risk of getting discriminated just by their ethnicity. This effect even if critical from a fairness perspective, it might appear unnoticed on the model overall loss functions.  

Furthermore, the problem gets more aggravated when dealing with intersectional fairness or the concatenation of a protected attribute with another category. In this case, the cardinality of the categories grows exponentially, leaving groups with less statistical weight, thus allowing the algorithms to make even un-fairer encodings \gourab{I would prefer to use ``even less representative encoding" instead}


Another alternative can be dropping protected and sensitive features, but this can lead do sub-optimal results, the question that arises is: \textit{Can we utlize a protected attribute and achieve both a performing and fair solution?}


Even though fairness in machine learning can be crucial, and there have been an enormous effort from the research community to design  new algorithmic methods, from an applied perspective it's a desiderata that is often optional to have.
A common assumption is that methods that improve the accuracy-fairness trade off may necessitate from complex methods and difficult choices \cite{negligible2021,heidari2019fairness,friedler2018comparative,kearns2018empirical}.


While there are methods that implement "fair algorithms", they require to modify the long-stablished, well tested and performing machine learning pipeline to include newly developed and untested software\cite{zafar2017fairness,zafar2017parity,zafat2017fairnessDisparate} \gourab{Explain ``newly developed and untested software" with more details and add criticisms to justify their impracticality}. We democratize fairness allowing all data scientist and developers to improve the fairness on their machine learning projects by providing an accessible and low friction method to improve discrimination. The methods that we use on this paper are all publicly tested and developed in a user friction minimal way, the Python packages used for the testing are all well known ($\texttt{scikit-learn}$, $\texttt{catboost}$ and $\texttt{category\_encoders}$) and conform within the traditional ML pipeline and are deployment and production ready. 
\gourab{As far as I understand, you are proposing regularization in target encoding as an alternative to the prior fairML works, stressing upon the fact that this method is more practical and low friction. Then, we should give good arguments/analyses on (i) why prior fairML works are high friction and less practical (are there evidences suggesting this?), (ii) can regularized target encoding give fairness-accuracy trade-offs comparable to the prior works on fairML?}

While there are open source packages and methods developed that implement "fair machine learning" \cite{2018aequitas,bird2020fairlearn,aif360-oct-2018}, their usage in the long-stablished, well tested and performing machine learning production pipeline is yet untested. 
%\gourab{Explain ``newly developed and untested software" with more details and add criticisms to justify their impracticality}

We re-evaluate traditional target encoding over-fitting regularization as methods to reduce both induced discrimination in the encoding of categorical variables. 
Even though fairness in machine learning can be crucial, and there have been an enormous effort from the research community to design  new algorithmic methods, from an applied perspective it's a desiderata that is often optional to have.
A common assumption is that methods that improve the accuracy-fairness trade off may necessitate from complex methods and difficult choices \cite{negligible2021,heidari2019fairness,friedler2018comparative,kearns2018empirical}.



Some conclusion about figure \ref{fig:regularization}.
\begin{itemize}
    \item Gaussian regularization affects both accuracy and fairness. Smoothing regularization has negligible effects on both metrics.
    \item One Hot Encoding systematically achieves less fair results (more discriminant), and it does not necessarily achieve a better model performance than using statistical target encoding. 
    \item Little adjustments on the regularization of Gaussian Noise almost achieve equal disparate treatment fair solutions with a negligible impact on model performance.
    
    \item Gaussian regularization minimizes fairness, independent of the size of the minority group. While smoothing only affects in case of groups with light statistical weight.
    
    \item Smoothing  impact in the model overall loss function is negligible, as it's effect on small groups becomes unnoticed in the presence of larger groups. This is not the case for fairness, where minority groups such as \textit{Asian}, \textit{HispanicMarried} for Compass data and \textit{Amerindian} or \textit{MexicanFemale} are benefited in the case of disparate mistreatment. 
\end{itemize}


\section{Discussion}

In this section we overview some discussion topic that the problem of encoding categorical attributes arises and whose solutions remains unknown to the community. 

\steffen{I do not see value here, other than the one point that could be moved to conclusion}

\subsection{How to handle properly the encoding of sensitive data?}

Encoding sensitive and protected attributes is a common need in data scientist and data engineering tasks. Even if there are a plethora or encoding methods that can deal with protected categories, common guidelines that study the benefits and drawbacks of this techniques when dealing with protected and sensitive attributes are still in-existent.

\subsection{Are there encodings that are more compliant with EU antidiscrimination law?}

\steffen{I doubt that this is a meaningful question}

It has been proven that different encoders optimize different metrics \cite{quantile2021}, these paper recently found that there are trade-offs on accuracy-fairness and opens the question on \textit{what are the encoders that are more compliant with antidiscrimination law?}

\subsection{Improving on the pre/post processing or in the modeling}
In recent years we have seen algorithmic methdos aiming to improve fairness in AI systems from many perspectives: data collection, pre-processing, modeling, post-procesing \ldots

\steffen{This sounds more like a --- very good --- conclusion than a point for discussion}

In our work we have provided evidence that in already implemented machine learning production pipelines we can improve fairness by introducing minimal changes on the regularization at the pre-processing stage. Allowing data scientist and ML engineers to improve disparate discrimination between groups in a low user-friction way. 


we started by comparing the two most popular encoders in aspects of model performance and disparate treatment fairness in the well-known Pro-Publica dataset of Compass.
Furthermore, we studied how to regularize statistical Target Encodings, noticing that from the two most typical regularization methods smoothing does contribute little to fairness and model performance, but adding Gaussian noise can reduce significantly the discriminatory power of the algorithm while maintaining accuracy.

We were able to provide empirical evidence over the Compass dataset, that by regularizing with Gaussian noise we were able to reduce significantly fairness with an almost negligible drop-in model performance.


\todo{Your average Joe: the role of the practitioner}

@All: I'm not sure if here, but we really need to have a dedicated section where we argue for why it's important to keep the average ML/DS practitioner in mind. What comes to mind here:

\begin{itemize}
    \item Fair solutions don't have to be complex: Would cite papers/arguments (thinking, e.g., of Cynthia Rudin's work) that propose simple, existing solutions to tackle fairness. In practice, this means that possible solutions can be already available and familiar to your average practitioner, reducing the implementation costs, which are key within business settings (@Carlos, we can cite your ECB paper here for example - the average practitioner is also a key stakeholder for fairness). This, in turn, should increase the likelihood of adoption beyond academic circles. The clearest example, though I'm not sure if we should mention it, is how difficult it was for Carlos to implement \cite{zafar2017fairness}'s fair logit code (very certain that leading tech-oriented companies don't use Python 2 for their tools). 
    
    \item Algorithmic anti-discrimination law is not there yet: I would stress that, at least in the case of the EU, we're only at the beginning of setting up the regulatory framework (maybe cite the recent memos Commission's AI team - GDPR is not enough). I would argue that in the long-term regulating fairness will be on a industry-specific or even case-by-case basis, especially when it comes to proving discrimination or unfair treatment - cite \cite{Hacker2018_TeachingFairnessToAI} arguing that most algorithmic discrimination will be indirect and \cite{Wachter2021_FairnessCantAutomate} that discrimination cases will have to be on case basis to work under current EU and EU-member laws. In practice, what this means is that the people building and implementing these models will become crucial in preventing and/or (dis)proving algorithmic discrimination as this level of granularity can't be implemented at large scale. I would argue that something similar to the Basel agreement among leading banks and the credit modeling (read capital minimum requirements) will occur, where banks can either model credit using simple but conservative models provided by the ECB and agreed upon in Basel II (or III) or develop their own models as long as they document all steps and are able to defend them to the ECB. Under this approach, credit risk modelers are key. It can take up to a year to develop, defend and approve one of these models (only big bank can afford this)... maybe fair encoding could be provided as a benchmark practice?  
    
    \item Categorical data needs to be made machine readable: we argued this before. Even your Stata-running social scientist is taught to encode categories into dummy variables (see, e.g., \cite{Wooldridge2015_IntroductoryMetrics}).  
\end{itemize}

All of this considered, studying encoding from a fairness perspective is both of interest to our field and important in practice: it is not an exaggeration to assume that your average practitioner will first try to solve the fairness problem using techniques that she knows rather than trying to implement code that was never designed for deployment.

\subsection{Target encoding}
\begin{table}[h]
\begin{tabular}{ll}
\hline
Notation                 & Meaning                                           \\ \hline
$\D$                     & dataset $\D=\{(x_0,y_0)\ldots (x_n,y_n)\}$        \\
$x_{i,j}$                & value of attribute $j$ of data item $i$           \\
$x_{:,j}$                & entire feature $j$ column vector.                 \\
$P(X,Y)$                 & joint underlying distribution                     \\
$X^\star$                & encoded attribute                                 \\
$\mu_X$                  & mean of a random variable.                        \\
$\sigma_X$               & standard deviation of a random variable.          \\
$N(\mu,\sigma^2)$          & Gaussian distribution                             \\
$\mathbb{N}$             & the set of natural numbers                        \\
$\mathbb{R}$             & the set of real numbers                           \\\hline
\end{tabular}
\caption{\label{tab:notation} Notation used throughout the paper \sr{I think this table is not used/not consistent with notation in text}}
\end{table}


\section*{Computational Performance}
All computing performance experiments were run on the 4 vCPU's server of 15GB of RAM. Values are estimated out of a 100 iterations sample and using default \texttt{scikit-learn} and \texttt{category-encoders} hyperparameters. 

 \cite{scikit-learn,category_encoders}.

\begin{table}[h]
\begin{tabular}{llll}
                                                          & \textbf{LogisticRegression} & \textbf{DecisionTree} & \textbf{Gradient Boosting Classifier} \\ \hline
\multicolumn{1}{l|}{\textit{One Hot Encoding}}            & 1250 $\pm$ 93                 & 660 $\pm$ 60            & 6046 $\pm$ 459                          \\
\multicolumn{1}{l|}{\textit{Target Encoding (smoothing)}} & \textbf{644 $\pm$ 44}         & \textbf{259 $\pm$ 2}   & 2390 $\pm$ 89                \\
\multicolumn{1}{l|}{\textit{Target Encoding (Gaussian)}}  & 752 $\pm$ 84                  & 282 $\pm$ 3           & \textbf{1580 $\pm$ 16   }                    
\end{tabular}
\caption{Computational performance comparison across different encoding methods. Values in milliseconds (ms).}
\label{tab:performance}
\end{table}

From table \ref{tab:performance}, we can see that target encodings consistently achieves a more computational performant solution.


Ioanna Papageorgiou: Some first thoughts: You are not extreeeemely precise in the first 2 sentences but almost!So I think it's more than fine as the focus of the paper is not legal. It might be better like this cause if you try to be more precise you may fall into mistakes. 
                                                                   
Just for your knowledge about the "(e.g.... )": Out of the four examples you mentioned just the first 2 are explicitly forbidden by the law (i.e. sexual orientation and ethnicity)
About the other 2 (zip code & marital status) the Eu anti discrimination law doesn't say anything, but their use for unfair treatment can be illegal, in case of an indirect discrimination 
Zip code for example has been proven in some court cases to correlate with Ethnicity and be illegal as indirect discrimination 
BUT not always. So on the one hand there is somehow a balance in your examples cause two of the attributes are explicitly forbidden and the other two might give rise to indirect discrimination 
But just to be clear that the law does not say that you can not treat two individuals differently based on their zip code or marital status. So if a model uses marital status it is not as such prohibited by the law.   I don't know whether zip code and marital status are specifically useful for your analysis, cause I haven't read the whole paper yetIf yes, then keep it as it is , it's not a big problem and it also does make sense.
If it is irrelevant for your technical approach which attributes you will mention as an example here, then it might be safer to mention some of the following attributes: ethnicity, gender, sexual orientation, age , religion


Ioanna Papageorgiou: I don't get the citation N.10 . The 11th is correct, I might preferably specify the art. 21 of the Charter - where the right to non discrimination is stipulated - and not just Charter of Fundamental rights.   Furthermore I would cite the following EU antidiscrimination directives :  Council Directive 2006/54/EC of the European Parliament and of the Council of 5 July 2006 on the implementation of the principle of equal opportunities and equal treatment of men and women in matters of employment and occupation (recast), OJ L 204; Council Directive 2000/78/EC establishing a general framework for equal treatment in employment and occupation [2000] OJ L303/16; Council Directive 2000/43/EC implementing the principle of equal treatment between persons irrespective of racial or ethnic origin [2000], OJ L180/22; Council Directive 2004/113/EC of 13 December 2004 implementing the principle of equal treatment between men and women in the access to and supply of goods and services, OJ L 373

\steffen{any suggestions for better terminology and `induced first/second-order discrimination'?}
\textcolor{red}{JA: Discrimination is technically a legal term and only splits into direct and indirect so I wouldn't introduce these orders as they're not legally defined. Maybe encoding-specific and variance-specific unfairness? TBD.}
\gourab{I would avoid naming them unless we explicitly define them both. Rather we can refer to them based on their characteristics.}
\carlos{From the uncertainty field there are two types: epistemic refering to the lack of data and aleatoric, refering to inherently random proces. We could use the same terminology. At least for me 2order = epistemic fairness}
\steffen{At this point, we have introduced and defined the problem, but now we need to sketch in the introduction what we will deliver in this paper to remedy the issue. What would be a natural approach that we could also use as part of this narrative?
\\
1. demonstrating that what is said above does indeed occur\\
2. regularizing\\
anything else? how do we frame the analysis?}



%With regard to \emph{(ii)}, categorical attributes, and especially those with many categories, tend to occur in imbalanced distributions.
%Such imbalance may become even more pronounced, when modeling  merges several categorical attributes into one, a strategy that often  improves model quality substantially \cite{howtowinKaggle}, but that may also  increase effects of intersectionality \steffen{any citation for this?}. 
%Thus, beyond the primary problem of unfairness possibly acquired from the use of protected attributes, which we call \emph{induced first-order discrimination}, the secondary problem of \emph{induced second-order discrimination} may imply unfairness  because of large variance found in sampling small groups. \steffen{any suggestions for better terminology and `induced first/second-order discrimination'?}
%
%The interplay of encoding \emph{(i)} with induced first- and second order discrimination \emph{(ii)} and their effects on the antagonistic trade-off between model quality and fairness have not been studied in the literature, although they concern a machine learning practice that is ubiquitous, especially when personal data is involved.
%An exemplary use case can be done with the well known COMPAS dataset , whose goal is to predict the risk that a criminal defendant will re-offend.
%It's been established in the literature \cite{compass} that a criminal's ethnic was paramount when determining recidivism score, the numerical encoding of ethnics such as \textit{African-American} or \textit{Caucasian} is what we call \emph{induced first-order discrimination}. 
%Furthermore,  a \emph{induced second-order discrimination} can be found when encoding ethnics such as \textit{Arabic} that are fairly represented in the data, provoke a large sampling variance that ends in an almost random  and unrealistic encoding. 
%% Being able to distinguish between the two types of fairnes might not be trivial in many real cases.


%\gourab{TODO: Need a link to next paragraph}
%With regard to \emph{(i)}, most learning algorithms require a numerical encoding of attributes. Encoding categorical features to numerical has been extensively studied in the literature with  statistical methods first introduced in the mid 1950's \citep{high-cardinality-categorical,quantile2021,statisticallearning}.
%Since then, these methods have  been applied in a plethora of machine learning applications, with two of them being most widely used: One Hot Encoding and statistical Target Encoders \cite{quantile2021,category_encoders,catboost-encoder,pargent2021regularized}.
%\emph{One Hot Encoding} produces orthogonal and equidistant vectors for each category.  \cite{one_hot,natureOHE,quantile2021}.
%However, it  suffers from scalability and sparsity when dealing with high cardinality categorical variables \ref{sec:relatedwork} due to the creation of many orthogonal dimensions.
%\emph{Target Encoding} (or \emph{mean encoding}) \cite{quantile2021,high-cardinality-categorical,pargent2021regularized} works as an effective solution to overcome the issue of high cardinality of the categorical variable. In target encoding, categorical features are replaced with the mean target value of each respective category.\footnote{Target encoding methods have become an industry standard for high-cardinality categorical data \citep{quantile2021,pargent2021regularized,target_embedding} with algorithmic procedures being implemented in many open source packages \cite{sktools,category_encoders}. One of the most common is  \textit{category encoders} a Python package. It achieves up to 1 million downloads per month.  ({\url{https://pepy.tech/project/category_encoders}}) Category encoders is  the default encoding method in some high-performance open source software implementations such as \textit{catboost} \cite{catboost-encoder,hancock2020catboost,dorogush2018catboost} that has reached a total download of 33 millions.}




%\gourab{TODO: Structure like this. 1. Many earlier works on fair ML have looked into limited number of disjoint classes. However it is sometimes far from the reality (give examples with references) 2. Some works have transformed datasets with non-disjoint categories to disjoint ones by merging multiple attributes into one (like Af-male, Wh-female, etc.). 3. However, with this approach the general problem of class imbalance gets pronounced more (add references or forward references). 4. Thus we study the implications on fairness-accuracy trade-off by target encoding categorical attributes under intersectionality.}
%\gourab{By this point, a reader will forget what were (i) and (ii)? Replace them with representative terms and make them bold.}
%

%\gourab{Do these paper explicitly talk about these limitations of fairML?}
%\gourab{What do they mean by overly complicated methods or difficult choices? We must discuss this to motivate our approach.}
%Previous research work in fair algorithmic development might have been developed for researchers themselves rather for real life discrimination use cases.
%We operationalize fairness by providing an accessible, low friction and ready for production method to improve bias in AI systems. Previous work in fair machine learning has been either illustrative \cite{zafar2017fairness,zafar2017parity,zafat2017fairnessDisparate}

%\gourab{I think we should remove the following paragraph and directly list the contributions}
%\steffen{what should `illustrative' mean?}
%or not developed to be integrated with a long-stablished, well tested and performing machine learning production pipeline \cite{2018aequitas,bird2020fairlearn,aif360-oct-2018}
%The methods that we use on this paper are all publicly tested and developed in a user friction minimal way, the Python packages used for the testing are all well known ($\texttt{scikit-learn}$ and, $\texttt{category\_encoders}$) and conform within the traditional ML pipeline and are deployment and production ready.. 
%\steffen{I do not buy this `production ready'}

%\gourab{As far as I understand, you are proposing regularization in target encoding as an alternative to the prior fairML works, stressing upon the fact that this method is more practical and low friction. Then, we should give good arguments/analyses on (i) why prior fairML works are high friction and less practical (are there evidences suggesting this?), (ii) can regularized target encoding give fairness-accuracy trade-offs comparable to the prior works on fairML?}


%\steffen{I find the following paragraph to be uninformative for the FAcct conference audience. I would discard it}
%Improving fairness in machine learning projects has been a vibrant research and industry topic in recent years with many conferences published papers, workshops \cite{ecml2020biasworkshop,specialIssueFairness} and open source software development packages \cite{2018aequitas,bird2020fairlearn,aif360-oct-2018}. Due to far-reaching impact on society and individuals of algorithms that are employed in many scenarios including central banking, education, healthcare, and public policy \cite{mougan2021desiderata}. The fairness research community has made an enormous effort to understand, mitigate and account for bias in AI-decision making systems\cite{ntoutsi2020bias}. Various publications reconcile the information of relevant papers, create explainable fairness and bias taxonomies CITE.


%The fairness research community has made an enormous effort to understand, mitigate and account for bias in AI-decision making systems\cite{ntoutsi2020bias}.  A common expectation that limits much of this work and research is  the assumption that trade-offs between fairness and accuracy may require overly complicated methods or difficult choices \cite{negligible2021,heidari2019fairness,friedler2018comparative,kearns2018empirical}.
%\gourab{Do these paper explicitly talk about these limitations of fairML?}

%\gourab{Cite art. 21 of EU fundamental rights charter \cite{EU_fundamentalrights} instead of gdpr.}

%Anti-discrimination laws \cite{gdpr} prohibits unfair treatment of individuals based on specific traits, also called sensitive or protected attributes (e.g., sexual orientation, ethnicity, marital status). These laws typically distinguish between two different notions of unfairness \cite{Barocas2016BigDD} namely, \textit{disparate treatment} and \textit{disparate impact}.  More specifically, there is disparate treatment with respect to a given sensitive attribute if the missclasification rates for groups of people have different values of that sensitive attribute.

%\cite{zafar2017fairness}, mitigate disparate treatment fairness by developing a decision boundary-based classifiers, which can be easily incorporated into their formulation as convex-concave constraints. In order to avoid high cardinality scenarios, they simplify by only consider a subset of offenders whose race was either black or white. While in our case we deal with all the different types of ethinicity up to 9 distinct values and increase the cardinality of problem by tackling intersectional fairness. 

%$This notion can be stated in a very intuitive way: \textit{two similar persons should not be treated differently solely because of a difference in a protected attribute}.

%Anti-discrimination laws \cite{gdpr} prohibit unfair treatment of individuals based on specific traits, which are also called sensitive or protected attributes (e.g., sexual orientation, ethnicity, zip codes, marital status), excluding their direct use in many applications. For other applications, protected and sensitive attributes can be utilized during the modeling. The usage of these attributes can improve the model predictive performance, at the cost of being highly discriminant.
%\gourab{TODO: Structure the following three paragraphs like this. 1. General motivations for fairness and the importance of categorical attributes. 2. Give the example on abundance of categorical attributes in COMPAS. 3. However, fair ML literature has largely ignored the fairness-accuracy implications of how the MLA interprets the categorical attributes. 4. (just 1-2 lines with forward reference) We find that it is quite important and plays a huge role in fairness-accuracy dynamics of MLA.}
% FIRST PARAGRAPH: Linking fairness in ML, protected categorical attributes, and datasets with personal info. How our contribution is exploring an area overlooked in prior work.
% context of our work


%Anti-discrimination laws \cite{gdpr,EU_fundamentalrights} prohibit unfair treatment of individuals based on \emph{sensitive attributes}, also called as \emph{protected attributes} (e.g., sexual orientation, ethnicity, zip codes, marital status). 
%Sensitive attributes may be pivotal to the quality of machine learning models and poor quality models may themselves cause unfairness  \cite{DBLP:journals/ail/ZliobaiteC16}, however, the explicit usage of sensitive attributes raises questions about how to reconcile quality of models and fairness.
% why is our work relevant and important
%In this paper, we study how the use of categorical attributes relates to the trade-off between model quality and fairness. Categorical attributes are ubiquituous in datasets with personal information, e.g.\ the famous COMPAS dataset \cite{compass} comes $11$ ($\approx 75\%$) of its features being categorical (more details in \ref{sec:experiments.compass}).
%\gourab{add forward references wherever needed}
%why is there not a trivial solution
%Modeling a machine learning problem with categorical attributes typically requires pre-processing and encoding the data in ways that are, \emph{(i)}, amenable or machine-readable and, \emph{(ii)}, most useful for exploitation by the machine learning algorithm.
%\gourab{TODO: Structure the following like this. MLA require encoding of categorical attributes. A widely used method is one-hot. However, problems with one-hot: orthogonal, equidistant, not scalable. Another way is target encoding, examples, benefits, evidences suggest it has become an industry standard.}
% SECOND PARAGRAPH: Numerical encodings, One-hot, Target
% 1. Machine readability -> numerical encoding

%
% 2. Two most widely used encodings: One hot, target


%
%\sr{Confusion here. EO is the fairness notion, and disparate treatment is the metric. Be consistent, or use only one name for both!}
%
%As a measure of unfairness, we use the estimation of the \textit{equal opportunity fairness (EOF)} metric (\ref{def:eo}), also known as disparate treatment %\sr{confusion introduced here, why using two names, but eq. (8) use EOF?} % which arises when a decision-making system provides different outputs for groups of individuals with the same values of non-protected attributes but different values of protected attributes 
%\cite{zafat2017fairnessDisparate}. 

==> mysc/CheckList.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} These were highlighted in the Experiments and Conclusion sections.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerNA{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} A link is provided in the Introduction section.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} This is mentioned in the beginning of the Experiments section.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} This is mentioned in the beginning of the Experiments section.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> mysc/oldExperiments.tex <==
\section{Experiments} 
\label{sec:experiments}
In this section, we aim to evaluate the implications of model accuracy and fairness when encoding categorical protected attributes in real datasets for one-hot encoding and target encoding and also compare against the case of not including the protected attribute in the training data. Furthermore, we study the impact of target encoding regularization and extend our experiments towards an inter-sectional fairness case.

In the first experiment, we tackle the fairness implications from the irreducible bias, by comparing two large groups. In the next experiment, we go through the reducible bias case. Finally, in the last experiment, using intersectional fairness, we improve the model performance but also make a more discriminant model for both bias scenarios. We provide empirical evidence of the implications of encoding protected categorical attributes over two datasets: COMPAS and Law School Admission Council.\footnote{Experiments on Law School Admission Council dataset are reported in the appendix (cf. Section~\ref{sec:appendix}).}

\subsection{COMPAS}
\label{sec:experiments.compass}

The scenario we want to address is characterized by datasets that display categorical features with a high cardinality of sensitive attributes in a binary classification problem. We make use of the COMPAS dataset \cite{compass}. COMPAS is an acronym for Correctional Offender Management Profiling for Alternative Sanctions, which is an assistive software and support tool used to predict the risk that a criminal defendant will re-offend. The dataset provides a category-based evaluation labeled as high risk of recidivism, medium risk of recidivism, or low risk of recidivism. We convert this multi-class classification problem into binary classification combining the medium risk and high risk of recidivism vs. low risk of recidivism. The input used for the prediction of recidivism consists of 11 categorical features, including gender, custody status, legal status, assessment reason, agency, language, ethnicity, and marital status. The sensitive feature that we will be looking at is \textit{Ethnic} for the single discrimination, whose protected group will be the most represented group: African-American (cf. Figure~\ref{fig:pieCompas}).


For intersectional fairness, we created the variable \textit{EthnicMarital}, engineered by concatenating \textit{Ethnic} and \textit{Marital} status. This new feature has a high cardinality of 46 distinct values (cf. Figure~\ref{fig:pieCompas}). The most predominant category is \textit{African-American Single}, and it will be the protected group (cf. Figure~\ref{fig:pieCompas}) for the intersectional fairness case. To compare disparate treatment between groups we will make use of  \textit{Caucasian Married} as the reference group. It is worth noting that the contribution of the features to the model performance, based on feature importance explanation mechanism\cite{shapTree,ribeiro2016why,christoph_molnar2019_interpretableML,desiderataECB}, is highly relevant. %In Figure \ref{fig:pieCompas}, the categories of the protected attributes are represented. 
The available data is split into a 50/50 stratified train/test split, maintaining the ratio of each category between train and test set.


\begin{figure}[ht]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.2\linewidth]{images/ethnicPie.eps}
  \caption{\textit{Ethnic} categories distribution}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.2\linewidth]{images/ethnicmaritalPie.eps}
  \caption{Intersectional fairness \textit{EthnicMarital} categories distribution}
\end{subfigure}
\caption{Distribution of the protected attribute categories to be encoded and regularized for the COMPAS data \cite{compass}. %Predominant \textit{Ethnic} categories are \textit{African-American} and \textit{Caucasian}. For the intersectional fairness case (b), the number of categories is increased to 46 distinct groups.
}\label{fig:pieCompas}
\end{figure}

In Figure~\ref{fig:pieCompas}, we show the distributions of the ethnic groups (a) and the intersectional groups of ethnic and marital status (b). There are two groups (\textit{African-American} and \textit{Caucasian}) that account for the $80\%$ of the data, while there are less represented groups such as Asian or Arabic that have a less significant statistical weight. For the intersectional fairness case, the number of groups increases, making room for more distinct, disparate, and imbalanced groups. 



\subsection{Choice of metrics and models}
\label{sec:methodology.metrics}
\subsubsection{Fairness metrics}

We have selected three fairness metrics to showcase the fairness impacts of encoding categorical protected attributes, the three metrics have in common that the lower the value the more fair the model is. 

As we are in high cardinality categorical scenarios ($\sim 10$ distinct values of the protected attribute). We calculate the overall fairness $\mathcal{L}$ of the model $f_\theta$ on data of interest $X$ given a fairness metrics $\ell$, reference group $(j)$ and rest of groups $(i)$ as:
\begin{equation}
    \mathcal{L}(f,X) = \sum_{i \in X\setminus \{j\}} |\ell(\hat{f}(X_j),\hat{f}(X_i)) |
\end{equation}
\begin{itemize}
    \item  \textbf{Equal opportunity fairness.} Following \citet{DBLP:conf/nips/HardtPNS16}'s emphasis on ensuring fair opportunity instead of raw outcomes (it also remains a guiding principle in domains like credit scoring \cite{bigdata_potus,bigdata_potus1}), we choose \emph{equal opportunity} (EO) as a fairness notion and use the metric {\it disparate treatment} (difference between the true positive rates) to measure unfairness, which is estimated using the disparate treatment metric \cite{zafat2017fairnessDisparate}---hence, for simplicity, we refer to the interplay of these concepts as the \textit{equal opportunity fairness (EOF)} metric. The value is the difference in the True Positive Rate (TPR) between the protected group and the reference group: %reference group and the group whose \textit{disparate treatment} we want to evaluate. 
%This metric intuition can be understood as  \emph{equality of opportunity} \cite{hartdt_equality,negligible2021}. We measure TPR disparity as the difference between the recall attained by a model for one group of interest (such as \textit{Caucasian} individuals) and the model’s recall for the reference group \textit{African-American}.

    \begin{equation}\label{eq:TPR}
    \text{TPR} = \frac{\text{TP}}{\text{TP + FN}} \hspace{2cm} \text{Equal Opportunity Fairness} = \text{TPR}_j - \text{TPR}_i
    \end{equation}

    A negative value in (\ref{eq:TPR}) is due to the worse ability of a Machine Learning model to find actual recidivists for the protected group (i) in comparison with the reference group (j).

    
    \item Statistical Parity (Strong Demographic Parity): The difference between favourable out-comes received by the unprivileged group and privileged group ~\cite{kamishima2012fairness,DBLP:conf/icml/ZemelWSPD13,DBLP:conf/kdd/FeldmanFMSV15,DBLP:conf/kdd/Corbett-DaviesP17}. SDP ensures that a fair decision does not depend on the sensitive attribute regardless of the classification threshold used  \cite{DBLP:conf/uai/JiangPSJC19,DBLP:conf/aaai/ChiappaJSPJA20} $d(P(f_\theta(X)|Z=i),P(f_\theta(X)|Z=j))=0$ where $d(\cdot,\cdot)$ is a distance function. In this work we use the Wasserstein distance as a measure between the two probabilistic distributions.
    
    \item Average Absolute Odds (Equalized Odds): The sum of the absolute differences between the True Positive Rates and the False Positive Rates of the unprivileged group plus the same ratio for the  privileged group.
    
    \begin{equation}\label{eq:AAO}
    \text{FPR} = \frac{\text{FP}}{\text{FP + TN}} \hspace{2cm} \text{Average Absolute Odds} = |TPR_j - FPR_j| + |TPR_i - FPR_i|
    \end{equation}

\end{itemize}
\subsubsection{Model performance} For model performance metrics, as we are in a binary classification scenario, we use the Area Under the Curve (AUC)---a  metric that illustrates the diagnostic ability of a binary classifier system as its discrimination threshold is varied \cite{statisticallearning}. This metric is less susceptible to class imbalance than accuracy or precision and also accepts soft probabilities predictions. % is an adequate candidate for our problem. For less technical readers is worth noting that 
An AUC of 0.5 is equal to doing random predictions, which can be used as a baseline for interpreting the model performance results. Previous work on fair machine learning experiments on COMPAS have focused on using accuracy as a performance metric \cite{zafat2017fairnessDisparate,zafar2017parity,zafar2017fairness}, but given the target ratio of the full dataset of COMPAS $(70:30)$, we consider accuracy to be a less informative measure of model performance. 

\subsubsection{Machine learning algorithms} As classification estimators, we experiment with a linear regression model, a decision tree model, and a gradient boosting decision tree. All models are trained on the training set. These three models provide examples of a model with large bias (the linear regression model), a model with large variance (the decision tree model), and an extensively used and with state-of-the-art performance model (gradient boosting decision tree) \cite{supervised_learning_algorithms,gbm_travel,gbm,gbm_nn,get_bristol}.


\subsection{Irreducible bias}
\label{exp:first}

The irreducible bias that is induced while encoding categorical features is due to different posterior probabilities among groups. It can be observed for large groups, where instead reducible bias due to variance is low. For this case, we will choose the two largest groups in the COMPAS dataset: \textit{African-American} and \textit{Caucasian}, (Figure~\ref{fig:pieCompas}). Recall that we will benchmark the trade-off between disparate treatment and AUC metrics while using two different encoding techniques (Section~\ref{sec:relatedwork}), with two different regularization techniques (Section~\ref{sec:methodology}) and three different estimators (Section~\ref{sec:methodology.metrics}). 

The ranges of the regularization hyperparameters are:  $\lambda \in$ $[0,1]$ for the width of the Gaussian noise regularization;  $m \in [0,10000]$ for the additive smoothing using the $m$-probability estimate function $\lambda(n_i) = n_i/(n_i+m)$ (see \cite{high-cardinality-categorical}). These hyperparameters will also be kept for the rest of the experiments for this dataset. 
The observed group target mean, namely $\hat{p}_i = n_{i, Y}/n_i$, is  $0.43$ for \textit{African-American}, and $0.25$ for \textit{Caucasian}.
%\sr{This statement does not make sense in English.}

\begin{figure}[ht]
    \centering
    \includegraphics[width=1.1\linewidth]{images/encCompassFull.eps}
    \caption{Comparing one-hot encoding and target encoding regularization (Gaussian noise and smoothing) for the Logistic Regression, Decision Tree, and Gradient Boosting classifiers over the test set of the COMPAS dataset. The protected group is \textit{African-American}. Reference group is \textit{Caucasian}. Red dots regard different regularization parameters: the darker the red the higher the regularization. Blue dot regards the one-hot encoding.}
    \label{fig:compas1}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/compassHyperGaussian.eps}
    \caption{Impact of the Gaussian noise regularization parameter $\lambda$ on performance and fairness metrics over the test set of the COMPAS dataset. In the left image the AUC of the protected group, reference group, and global over the regularization hyperparameter. On the right, the equal opportunity fairness variation throughout the regularization hyperparameter.
    %\sr{Remove TPR from the y-axis label} \sr{what classification model does this figure refer to?}  \sr{Describe what are the 'tot', 'African-American' and 'Caucasian' lines on the left plot. Not said/discussed in the text!} \sr{put space between the left and right plots}
    }
    \label{fig:hyperCompas}
\end{figure}

Figure \ref{fig:compas1} shows that the smoothing regularization effects are relevant for the logistic regression and negligible in both fairness and model performance for the other estimators. On the other hand, Gaussian regularization affects both metrics for all estimators. This is due to the adding of white noise to the data inhibiting learning. From Figure \ref{fig:hyperCompas}, we can see that there is an optimal value around $0.3$, where the disparate treatment has become negligible and the model performance has only slightly decreased. It is worth noting that performances for both groups have a negative slope. For the one-hot encoding (blue dot), the performance is very similar to the best target encoding (in terms of AUC). But, when the target encoder is correctly regularized (red dots) it achieves less or equal discriminant results consistently. 

\subsection{Reducible bias}
\label{exp:secondorder}

This second type of bias arises due to the large variance found when sampling small groups. To replicate this biased situation, from the most common ethnic group, \textit{African-American}, we sample a $\approx 0.002$ fraction, being the ratio of $50$ against $27,000$ samples (cf. Figure \ref{fig:pieCompas}). We treat this sampled group as it were a different category than the original \textit{African-American} group. Both come from the same distribution so if we had enough statistical mass for both of them, the encoding should be the same. We note that due to the stochastic nature of this sampling experiment, different randomization seeds will produce different results. For this split, the mean of the sampled group is $0.63$ while the reference group has a mean of $0.43$. The regularization hyperparameters are the same as in the previous experiment (Section~\ref{exp:first}).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/encTheory.eps}
        
    \caption{One-hot Encoding vs regularized target encoding (Gaussian and smoothing), comparing the reference group \textit{African-American} over a sample of the reference group. Smoothing regularization reduces group equal opportunity fairness with a negligible loss of AUC.
    Red dots regard different regularization parameters: the darker the red the higher the regularization. Blue dot regards one-hot encoding. Over tuning Gaussian noise hyperparameter causes a noticeable drop in performance. 
    %\sr{Rewrite caption as for / consistently with Figure 2}
    }
    \label{fig:theory}
\end{figure}


In Figure \ref{fig:theory}, we can see a logistic regression estimator that is fed encoded variables in the two different encoding ways. Non-regularized target encoding is more discriminant than one-hot encoding and the AUC is almost the same with negligible differences. For the smoothing regularization, it is curious to see that the model performance does not vary, but the fairness does so significantly. This is due to the regularization affecting only to categories with few samples and the global AUC being almost unaffected. For the Gaussian noise regularization, the effect is quite similar to the smoothing, but in case the $\lambda$ hyperparameter is over-tuned, the model performance drops significantly.
%Does smoothing effect only for categories with small data and Gaussian irrelevant of the data size? -- YES. Gaussian Encoder regularizes independent of the statistical mass of the minority category. While smoothing only for categories with few samples.

%Smoothing has a low impact on accuracy, while Gaussian has a progressive impact.



\subsection{Intersectional Fairness}
\label{exp:intersectional}

A common feature engineering technique that boosts model performance consists of concatenating two or more categorical features \cite{howtowinKaggle}. If the categorical features are protected attributes, the fairness problem is known as intersectional fairness \cite{RomeiR2014_DiscSurvey, Wachter2021_FairnessCantAutomate} (Section~\ref{sec:relatedwork.intersectional}). To provide evidence of the potential effects of encodings on intersectional fairness, we concatenate \textit{Ethnic} and \textit{Marital} status of the COMPAS dataset.  We select \textit{African-American Single} as the protected group and \textit{Caucasian Married} as the reference group. Both groups have enough statistical mass so the induced bias is not due to variance but rather it is irreducible bias. The group target mean is $0.46$ for \textit{African-American Single} and $0.10$ for \textit{Caucasian Married}. This is an increased difference between the two groups with respect to previous experiments when comparing single groups of \textit{African-American} and \textit{Caucasian}. 
 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/interCompasLinear.eps}
    \caption{Intersectional fairness case. One-hot Encoding vs regularized target encoding (Gaussian and smoothing), comparing \textit{African American Single} and \textit{Caucasian Married}.}
    \label{fig:regularization_inter}
\end{figure}

In Figure \ref{fig:regularization_inter}, we can see how feature concatenation can slightly boost the model performance to an AUC of $0.713$ using one-hot encoding against $0.709$ for the single group case (Figure~\ref{fig:compas1}). But we can also see how it worsen fairness: one-hot encoding achieves $-0.21$ of equal opportunity fairness (Figure~\ref{fig:compas1}) under single features, and $-0.28$ when using concatenated features. The Gaussian regularization overperforms smoothing in terms of fairness and model accuracy, not only the maximum values achieved but also at intermediate stages of regularization. This is not surprising, and, in general, feature concatenation can worsen fairness both on the side of irreducible bias (because $p_i$ and $p_r$ become more distant) and on the side of reducible bias (because $n_i$ becomes smaller).
